Planning Optical Networks for Unexpected Traffic Growth

A lightpath configuration algorithm considering a multi-period traffic model is presented and evaluated to a realistic German core network study.~Strategically exploiting BVT excess capacity, we show that offered traffic can be carried up to an additional five years in all traffic growth scenarios.

==> algorithm1.tex <==

\begin{algorithm}[htbp!]
\SetAlgoLined
\DontPrintSemicolon
\KwIn{$D_t$, $T_t$, $L_t$}    
\KwOut{$Next~period~Lightpaths~L_{t+1}$}
    \ForEach{$d_{i,j,t}$ in $D_{t}$}{
        
        $\tau_{i,j,t} \leftarrow T_{t}(i,j)$~
        $L_{i,j,t} \leftarrow L_{t}(i,j)$~
        
        $C_{i,j,t} \longleftarrow HeCSON$\supercite{Patri20}~
        
        \ForEach{$\lambda$ in $L_{i,j,t}$}{
             $\rho_{i,j,t}\cup\{\rho\} \subset C_{i,j,t}\ni BW_{\lambda}>=BW_{\rho}$
            
            $Sort~\rho_{i,j,t}~largest~DR~first$
            
            \ForEach{$\rho$ in $\rho_{i,j,t}$}{
                \If{$DR_{\lambda}<DR_{\rho}$}{
                $\tau_{i,j,t}~-= DR_{\rho} - DR_{\lambda} $~
                
                $Upgrade~\lambda~with~\rho$~
                
                $Update~Channel~Matrix$~
                
                \textbf{break}
                
                }
            }
            
        }
        $n_c \longleftarrow Eq.~$\ref{eq:ilp} 
        
        $Add~n_{c}~LPs~\forall~c~\in~C_{i,j,t}~to~L_{i,j,t+1}$
        
    }
    
    $Calculate~\eta_{NLI_\lambda}\forall~\lambda\in L_{t+1}$~
    
    $Update~Channel~Matrix$~
    
    $Find~SNR~\forall~\lambda\in L_{t+1}$~
    
    \textbf{return} $ L_{t+1} $
\caption{Upgrade and Add Lightpaths~(LPs)}
\label{algo:upgradeAdd}
\end{algorithm}


==> fllowchart1.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,895); %set diagram left start at 0, and has height of 895

%Flowchart: Terminator [id:dp6784388021447922] 
\draw   (161.3,3.57) -- (254.93,3.78) .. controls (267.09,3.81) and (276.94,12.03) .. (276.92,22.13) .. controls (276.89,32.24) and (267.01,40.41) .. (254.84,40.38) -- (161.21,40.17) .. controls (149.04,40.14) and (139.2,31.93) .. (139.22,21.82) .. controls (139.25,11.72) and (149.13,3.54) .. (161.3,3.57) -- cycle ;
%Flowchart: Process [id:dp07883249569474149] 
\draw   (106.7,65.56) -- (307.41,66.02) -- (307.27,127.64) -- (106.56,127.19) -- cycle ;
%Flowchart: Decision [id:dp38761554413019117] 
\draw   (207.99,156.55) -- (298.25,201.92) -- (207.78,246.88) -- (117.52,201.51) -- cycle ;
%Flowchart: Process [id:dp96717308302563] 
\draw   (97.74,276.42) -- (320.55,276.92) -- (320.41,338.55) -- (97.6,338.04) -- cycle ;

%Flowchart: Process [id:dp26952621236752106] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 189; green, 16; blue, 224 }  ,fill opacity=0.51 ][line width=1.5]  (554.48,229.51) -- (666.52,229.76) -- (666.35,301.96) -- (554.32,301.7) -- cycle ;
%Flowchart: Process [id:dp7270260326931108] 
\draw   (350.59,175.18) -- (420.59,175.34) -- (420.45,238.16) -- (350.45,238) -- cycle ;
%Straight Lines [id:da3212464660691814] 
\draw [line width=2.25]    (205.6,37.78) -- (205.54,61.91) ;
\draw [shift={(205.53,66.91)}, rotate = 270.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da5087254541448747] 
\draw [line width=2.25]    (208.05,127.42) -- (208,151.55) ;
\draw [shift={(207.99,156.55)}, rotate = 270.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da9697292038593301] 
\draw [line width=2.25]    (207.78,246.88) -- (207.73,271.01) ;
\draw [shift={(207.72,276.01)}, rotate = 270.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da7923231947615141] 
\draw [line width=2.25]    (208.51,335.29) -- (208.46,359.42) ;
\draw [shift={(208.44,364.42)}, rotate = 270.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Flowchart: Terminator [id:dp4809358013254865] 
\draw   (18.69,183.91) -- (76.67,184.04) .. controls (84.21,184.06) and (90.29,193.07) .. (90.27,204.17) .. controls (90.24,215.27) and (84.12,224.26) .. (76.58,224.24) -- (18.6,224.11) .. controls (11.06,224.09) and (4.97,215.08) .. (5,203.98) .. controls (5.03,192.88) and (11.15,183.89) .. (18.69,183.91) -- cycle ;

%Straight Lines [id:da4164049691173626] 
\draw [line width=2.25]    (355.93,203.41) -- (303.25,202.05) ;
\draw [shift={(298.25,201.92)}, rotate = 361.49] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Flowchart: Decision [id:dp4224841532390746] 
\draw   (489.35,282.32) -- (575.19,352.51) -- (489.03,422.32) -- (403.19,352.12) -- cycle ;
%Straight Lines [id:da7627177227821822] 
\draw [line width=2.25]    (117.52,201.51) -- (95.35,202.32) ;
\draw [shift={(90.35,202.5)}, rotate = 357.90999999999997] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Flowchart: Decision [id:dp6036806389789613] 
\draw   (208.47,363.68) -- (288.64,427.76) -- (208.18,491.48) -- (128.02,427.4) -- cycle ;
%Flowchart: Process [id:dp6961303398876826] 
\draw   (107.19,519.44) -- (330,519.94) -- (329.86,581.57) -- (107.05,581.06) -- cycle ;
%Straight Lines [id:da10870857515352217] 
\draw [line width=2.25]    (208.58,491.08) -- (208.53,515.21) ;
\draw [shift={(208.52,520.21)}, rotate = 270.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Flowchart: Decision [id:dp3540433075684051] 
\draw   (210.17,602.22) -- (308.17,679.22) -- (209.83,755.78) -- (111.83,678.78) -- cycle ;
%Flowchart: Process [id:dp10126178777355554] 
\draw  [fill={rgb, 255:red, 65; green, 117; blue, 5 }  ,fill opacity=0.63 ] (98.13,769.69) -- (321.07,770.19) -- (320.82,882.51) -- (97.87,882) -- cycle ;
%Flowchart: Process [id:dp28089030890613653] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.3 ] (363.56,625.03) -- (588.25,625.54) -- (588,737) -- (363.31,736.49) -- cycle ;

%Flowchart: Process [id:dp7043292133429531] 
\draw   (365.87,439.04) -- (672.3,439.73) -- (672,574) -- (365.57,573.3) -- cycle ;
%Curve Lines [id:da6185425080363103] 
\draw [line width=2.25]    (97.15,811.43) .. controls (62.54,811.35) and (47.27,687.29) .. (108.16,679.38) ;
\draw [shift={(113,679)}, rotate = 538.4100000000001] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da48022195495519115] 
\draw [line width=2.25]    (209.31,751.68) -- (209.26,766.68) ;
\draw [shift={(209.24,771.68)}, rotate = 270.18] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da538200643499215] 
\draw [line width=2.25]    (308,679) -- (359,679.91) ;
\draw [shift={(364,680)}, rotate = 181.02] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Flowchart: Off Page Connector [id:dp5155428263991446] 
\draw   (447.25,768.2) -- (503.25,768.32) -- (503.19,791.07) -- (475.18,796.26) -- (447.19,790.95) -- cycle ;

%Flowchart: Off Page Connector [id:dp004686705165980243] 
\draw   (76.83,453.38) -- (77.09,397.38) -- (99.84,397.49) -- (104.96,425.51) -- (99.58,453.49) -- cycle ;
%Curve Lines [id:da6895242263851544] 
\draw [line width=2.25]    (490.35,280.32) .. controls (488.97,252.33) and (419.06,265.03) .. (382.31,240.85) ;
\draw [shift={(378.45,238.07)}, rotate = 398.24] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Curve Lines [id:da9188787516367567] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (616,227) .. controls (615.58,195.48) and (517.51,196.95) .. (424.75,200.02) ;
\draw [shift={(420.51,200.16)}, rotate = 358.07] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Curve Lines [id:da3268449209124731] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (576.19,352.51) .. controls (573.95,352.01) and (614.66,373.13) .. (615.97,308.09) ;
\draw [shift={(616,304)}, rotate = 449.72] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da31840688003863993] 
\draw    (104.02,428.44) -- (128.02,428.5) ;
\draw [shift={(130.02,428.5)}, rotate = 180.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da43392559277047793] 
\draw [line width=2.25]    (211.67,581.69) -- (211.6,599.69) ;
\draw [shift={(211.59,604.69)}, rotate = 270.21] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da7189770865544052] 
\draw [line width=1.5]    (476,737) -- (475.33,766.26) ;
\draw [shift={(475.24,770.26)}, rotate = 271.31] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (11.61,-5.58) -- (0,0) -- (11.61,5.58) -- cycle    ;
%Curve Lines [id:da11554976266041117] 
\draw [line width=2.25]    (290.02,427.87) .. controls (336.34,427.97) and (304.06,499.19) .. (359.41,503.81) ;
\draw [shift={(363.85,504.03)}, rotate = 181.06] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Straight Lines [id:da7825811920328156] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (489.95,440) -- (489.96,425) ;
\draw [shift={(489.96,420)}, rotate = 450.01] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;

% Text Node
\draw (208.07,21.98) node  [font=\LARGE,rotate=-0.13] [align=left] {{\fontfamily{pcr}\selectfont \textbf{{\large Start}}}};
% Text Node
\draw (204.56,97.76) node  [font=\footnotesize,rotate=-0.13] [align=left] {\begin{minipage}[lt]{92.25900000000001pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\large {\fontfamily{pcr}\selectfont Init NW, RWSA, }}}\\{\large \textbf{{\fontfamily{pcr}\selectfont Traffic Model \ }}$\displaystyle T$\textbf{{\fontfamily{pcr}\selectfont  \ }}}\\{\large \textbf{{\fontfamily{pcr}\selectfont Time }}$\displaystyle t=0$}
\end{center}

\end{minipage}};
% Text Node
\draw (209.13,202.73) node  [font=\large,rotate=-0.13] [align=left] {\begin{minipage}[lt]{53.159pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\large {\fontfamily{pcr}\selectfont Is }}}\\{\large $\displaystyle t=t_{end}$}\\\textbf{{\large {\fontfamily{pcr}\selectfont ?}}}
\end{center}

\end{minipage}};
% Text Node
\draw (357.56,191.04) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {{\large \textbf{{\fontfamily{pcr}\selectfont t=t+1}}}};
% Text Node
\draw (569.44,245.54) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {{\large \textbf{{\fontfamily{pcr}\selectfont Upgrade }}}\\{\large \textbf{{\fontfamily{pcr}\selectfont Network}}}};
% Text Node
\draw (106.06,178.75) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.65310007697572pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont Yes}}}
\end{center}

\end{minipage}};
% Text Node
\draw (589.97,336.44) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.65310007697572pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont Yes}}}
\end{center}

\end{minipage}};
% Text Node
\draw (241.67,255.06) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.653100076975875pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\large No}}
\end{center}

\end{minipage}};
% Text Node
\draw (446.03,279.56) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.653100076975875pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont No}}}
\end{center}

\end{minipage}};
% Text Node
\draw (124.77,296.48) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{106.75184pt}\setlength\topsep{0pt}
\begin{center}
{\large {\fontfamily{pcr}\selectfont \textbf{Retrieve }}$\displaystyle L_{t} \ D_{t} \ T_{t}$}
\end{center}

\end{minipage}};
% Text Node
\draw (422.28,328.35) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{92.64184pt}\setlength\topsep{0pt}
\begin{center}
{\large {\fontfamily{pcr}\selectfont \textbf{Any link with }}}\\{\large $\displaystyle 75\%${\fontfamily{pcr}\selectfont \textbf{ filled }}}\\{\large {\fontfamily{pcr}\selectfont \textbf{slots?}}}
\end{center}

\end{minipage}};
% Text Node
\draw (163.06,402.59) node [anchor=north west][inner sep=0.75pt]  [font=\large,rotate=-0.13] [align=left] {\begin{minipage}[lt]{61.8205pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\fontfamily{pcr}\selectfont New }}$\displaystyle d_{i,j,t}$\textbf{{\fontfamily{pcr}\selectfont  }}\\\textbf{{\fontfamily{pcr}\selectfont in }}$\displaystyle D_{t}$\\\textbf{{\fontfamily{pcr}\selectfont ?}}\\
\end{center}

\end{minipage}};
% Text Node
\draw (141,520) node [anchor=north west][inner sep=0.75pt]  [font=\large,rotate=-0.13] [align=left] {\begin{minipage}[lt]{94.928pt}\setlength\topsep{0pt}
\begin{center}
{\large {\fontfamily{pcr}\selectfont \textbf{Retrieve }}}\\{\large $\displaystyle \tau _{i,j,t} \ L_{i,j,t} \ C_{i,j,t}$}
\end{center}

\end{minipage}};
% Text Node
\draw (162,632) node [anchor=north west][inner sep=0.75pt]  [font=\large,rotate=-0.13] [align=left] {\begin{minipage}[lt]{71.383pt}\setlength\topsep{0pt}
\begin{center}
{\large $\displaystyle \lambda $\textbf{{\fontfamily{pcr}\selectfont  in }}$\displaystyle L_{i,j,t}$\textbf{{\fontfamily{pcr}\selectfont  }}}\\\textbf{{\fontfamily{pcr}\selectfont {\large needs }}}\\\textbf{{\fontfamily{pcr}\selectfont {\large upgrade}}}\\{\fontfamily{pcr}\selectfont \textbf{{\large ?}} }\\
\end{center}

\end{minipage}};
% Text Node
\draw (99.24,773.52) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{151.25784000000002pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont Find }}$\displaystyle \rho \in \rho _{i,j,t}$}\\{\large \textbf{{\fontfamily{pcr}\selectfont Upgrade }}$\displaystyle \lambda $\textbf{{\fontfamily{pcr}\selectfont  with }}$\displaystyle \rho $}\\{\large \textbf{{\fontfamily{pcr}\selectfont Update Channel Matrix}}}\\{\large \textbf{{\fontfamily{pcr}\selectfont Update \ }}$\displaystyle \tau _{i,j,t}$}
\end{center}

\end{minipage}};
% Text Node
\draw (47.63,204.08) node  [font=\LARGE,rotate=-0.13] [align=left] {{\fontfamily{pcr}\selectfont \textbf{{\large Stop}}}};
% Text Node
\draw (177.03,754.56) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.65310007697572pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont Yes}}}
\end{center}

\end{minipage}};
% Text Node
\draw (326.97,668.56) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.653100076975875pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont No}}}
\end{center}

\end{minipage}};
% Text Node
\draw (468.24,773.24) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{13.362pt}\setlength\topsep{0pt}
\begin{center}
{\fontfamily{pcr}\selectfont \textbf{{\large A}}}\\
\end{center}

\end{minipage}};
% Text Node
\draw (365.23,457.32) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{204.816pt}\setlength\topsep{0pt}
\begin{center}
{\large {\fontfamily{pcr}\selectfont \textbf{Calculate }}$\displaystyle \eta _{NLI} \ ${\fontfamily{pcr}\selectfont \textbf{and SNR }}$\displaystyle \forall \ L\ in\ L_{t}$}\\{\large {\fontfamily{pcr}\selectfont \textbf{Remove blocked }}$\displaystyle L${\fontfamily{pcr}\selectfont \textbf{ from }}$\displaystyle L_{t}$}\\{\large {\fontfamily{pcr}\selectfont \textbf{Update Channel Matrix}}}\\{\large {\fontfamily{pcr}\selectfont \textbf{Update \ }}$\displaystyle \tau _{i,j,t}$}
\end{center}

\end{minipage}};
% Text Node
\draw (80.05,414.39) node [anchor=north west][inner sep=0.75pt]  [font=\large,rotate=-0.13] [align=left] {\begin{minipage}[lt]{15.487pt}\setlength\topsep{0pt}
\begin{center}
\textbf{{\large {\fontfamily{pcr}\selectfont A}}}\\
\end{center}

\end{minipage}};
% Text Node
\draw (186.85,501.13) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.65310007697572pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont Yes}}}
\end{center}

\end{minipage}};
% Text Node
\draw (337.94,461.47) node  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{35.653100076975875pt}\setlength\topsep{0pt}
\begin{center}
{\large \textbf{{\fontfamily{pcr}\selectfont No}}}
\end{center}

\end{minipage}};
% Text Node
\draw (364.51,630.09) node [anchor=north west][inner sep=0.75pt]  [rotate=-0.13] [align=left] {\begin{minipage}[lt]{151.25784000000002pt}\setlength\topsep{0pt}
\begin{center}
{\large {\fontfamily{pcr}\selectfont \textbf{Find }}$\displaystyle n_{c}${\fontfamily{pcr}\selectfont \textbf{ using Eq. 2}}}\\{\large {\fontfamily{pcr}\selectfont \textbf{Add }}$\displaystyle n_{c}${\fontfamily{pcr}\selectfont \textbf{ to }}$\displaystyle L_{i,j,t+1}$}\\{\large {\fontfamily{pcr}\selectfont \textbf{Update Channel Matrix}}}\\{\large {\fontfamily{pcr}\selectfont \textbf{Update \ }}$\displaystyle \tau _{i,j,t}$}
\end{center}

\end{minipage}};


\end{tikzpicture}
